Privacy-Aware Human Mobility Prediction via Adversarial Networks

As various mobile devices and location-based services are increasingly developed in different smart city scenarios and applications, many unexpected privacy leakages have arisen due to geolocated data collection and sharing. While these geolocated data could provide a rich understanding of human mobility patterns and address various societal research questions, privacy concerns for users' sensitive information have limited their utilization. In this paper, we design and implement a novel LSTM-based adversarial mechanism with representation learning to attain a privacy-preserving feature representation of the original geolocated data (mobility data) for a sharing purpose. We quantify the utility-privacy trade-off of mobility datasets in terms of trajectory reconstruction risk, user re-identification risk, and mobility predictability. Our proposed architecture reports a Pareto Frontier analysis that enables the user to assess this trade-off as a function of Lagrangian loss weight parameters. The extensive comparison results on four representative mobility datasets demonstrate the superiority of our proposed architecture and the efficiency of the proposed privacy-preserving features extractor. Our results show that by exploring Pareto optimal setting, we can simultaneously increase both privacy (45%) and utility (32%).

==> 3_proposedmodel/3_backup.tex <==
\section{Design of the Architecture}
\label{DoF}

In this section, we propose a semi-automated framework for evaluating the privacy and utility of any given dataset. 
Our framework consists of two main components responsible for \emph{Dataset Preprocessing} and \emph{Model Assessment}, connected via a command line interface for training and evaluating any model on any dataset illustrated in Figure \ref{fig:frameworkarch}. 
% Framework Architecture
% \begin{figure}[h]
%      \centering
%      \includegraphics[width=0.7\textwidth]{3_proposedmodel/2_framework_arch.png}
%      \caption{UML Class Diagram of the Framework Design}
%      \label{fig:frameworkarch}
% \end{figure}

The \textit{dataset} component is responsible for dataset-specific and generic preprocessing methods, such as transforming raw GPS data into user-week trajectories, as well as stratified train-test splitting. 
It allows the integration of any new spatial-temporal dataset, with parameters for temporal resolution, minimum points per trajectory, minimum trajectories per user, and test split ratio.
The \textit{model} component is responsible for defining neural network models that can be trained on different datasets, then be used to generate data, predict labels, and report performance metrics for comparison.
The \textit{model} component also handles further model-specific data preprocessing functionality, such as discretizing or transforming the spatial dimension into model features.
The command line interface provides three commands: \texttt{train}, \texttt{predict}, and \texttt{evaluate}, each of which is parameterized with one model and one dataset.
We utilize this framework in our experiments by training a generative model and a classifier model on the same dataset,
using the generative model to generate a synthetic dataset, and then evaluating the classifier model on the generated data and the original data and comparing its performance metrics.
In the next sub-sections, we describe each component in further detail.

\subsection{Dataset Preprocessing Module}
Raw GPS data collected from mobile devices tend to be noisy as well as sparse with location data missing for some subjects at some intervals~\cite{zheng2008learning}. 
They also tend to be high variance in the total span of time over which a single subject reports location data.
Preprocessing in the time dimension is necessary in order to produce a set of comparable trajectory examples for analysis, 
from many users' full location histories.

Our framework supports standard and custom (via inheritance) preprocessing methods per each dataset, using a base class called \texttt{Dataset}.
Dataset-specific subclasses must implement a \texttt{preprocess} method that reads the raw data from the source files and returns a dataframe with a user identification label column, a datetime column, latitude and longitude columns, and zero or more additional columns containing categorical variables. Then the \texttt{Dataset} base class provides a \texttt{to\_trajectories} method that converts the timestamped GPS locations into trajectories, assigning trajectory identifiers. By default, we define one trajectory as one user-week at ten minute resolution, and encode the day of week and hour of the day as categorical features. User-weeks with fewer than the specified minimum number of points are discarded, as well as users with fewer than the specified minimum number of trajectories. Then the base class also provides a \texttt{train\_test\_split} method that groups by trajectory identifiers and stratifies by user identification so that each user's weekly trajectories are randomly assigned to either the train or test set according to the specified probabilities, which we default to 70\% train and 30\% test.


\subsection{Model Assessment Module}

The \textit{Model Assessment Module} of our framework encompasses model-specific data preprocessing as well as model definition, training, prediction and evaluation functionality. 
We design a new loss function $L_{sum}$ of the core LSTM-AE model that enables it to be adaptable for both demands of the \textit{Model Assessment Module}, which can evaluate different datasets or report performance metrics, and requirements of an independent privacy-preserving mobility model, which can be utilized to attain a better balance between data utility and privacy protection in data sharing.

\subsubsection{Transformation Preprocessing}
First, we present the transformation preprocessing of the \textit{Model Assessment Module}.
Different from the steps in the \textit{Dataset Preprocessing Module,} the data preprocessing here is model-specific.
Preprocessing in the spatial dimension is commonly used to filter locations to a bounding box defining a city or region of interest
and then transforming continuous GPS coordinates by either standardizing and scaling them around a centroid position,
or by tessellating the space and encoding location as a discrete grid position.
For such spatial transformations, our framework provides classes for either min-max scaling GPS coordinates around a centroid, 
or for discretizing locations via the Geohash algorithm~\cite{morton1966computer} or via a rectangular grid of rectangular cells of user-defined size. 
These transformers can be utilized per model as appropriate for a given architecture and task.
Different models may also pad and/or truncate trajectory sequences to a configurable maximum length.

% Different selections for temporal and spatial resolution in the preprocessing phase will affect model performance and the privacy-utility trade-off,
% therefore our framework provides an evaluation module for measuring and comparing the impact of these selections.

\subsubsection{Problem Definitions}
Before describing our proposed LSTM-AE model in detail, we first give a brief problem definition of the trade-off between mobility data utility and privacy in terms of mobility prediction accuracy, de-identification efficiency and reconstruction data differences.

\textbf{Data Utility:}
Mobility datasets are of great value to understanding human behavior patterns, smart transportation, urban planning, public health issue, pandemic management, and etc.
As one of the most popular applications, mobility prediction not only can be analyzed to understand personalized location patterns, but also contributes to the large-scale communities services.
We focus on the capability of \emph{mobility prediction} (\emph{next location anticipation}) in this paper, and leverage the accuracy of the prediction as an important metric for quantifying the data utility.

\textit{Utility} (\textit{U}): the mobility prediction accuracy conducted by the extracted feature representation \textit{f}.

\textbf{Privacy Protection:}
With more and more intelligent devices and sensors are utilized to collect information about human activities, the trajectories also expose increasing intimate details about users' lives, from their social life to their preferences. The capability of de-identification of a data-sharing framework is important to balance the risks and benefits of mobility data usage, for all data owners, third parties, and researchers. We leverage the trajectory identification error as one of the privacy metrics to ensure the privacy-conscientious sharing of mobility data, alongside the data reconstruction loss.

\textit{Privacy I} (\textit{PI}): the differences between the reconstructed data $X'$ and the original data $X$, that is, information loss of the reconstructed data.

\textit{Privacy II} (\textit{PII}): the inaccuracy of the identification recognition, that is, the de-identification efficiency of the extracted feature representations \textit{f}.

A more obfuscated dataset will tend to perform better at preserving privacy, but worse at preserving utility, and vice versa, so monitoring these two performance metrics in tandem provides a way for
the user of the system to select the optimal privacy-utility trade-off for their use case, given their hyper-parameter selections.
Hence, our LSTM-AE model is designed to train a features Encoder $Enc_L(X)$ that could convey more information on the utility but less on privacy and investigate a better trade-off between them.
With a special designed loss function, the LSTM-AE model can also be utilized as an important portion of our \textit{Model Assessment Module} to assess and evaluate the utility and privacy performance of the target dataset. More details will be discussed in next sub-section.
%Mobility dataset shared to trusted or un-trusted services providers and the third parties can be utilized to attain personalized preferences. However, this shared mobility data also contains sensitive information, \textit{e.g.}., user identification and important activities. Obtaining better balance between data utility and privacy protection is an important task in data sharing. In this work, we quantify the privacy in two dimensions, \textit{Privacy I} and \textit{Privacy II}.

\subsubsection{Module Overview}
\label{section: module overview}

Fig.\ref{fig:architecture} presents the basic workflow of the proposed privacy-preserving representation learning architecture with adversarial learning (\textit{i.e.}, LSTM-AE) and the baseline LSTM model.
We aim to train an encoder $Enc_L(X)$ to automatically produce feature representations from the target time-series data, that these extracted features are optimized by simultaneously feeding into data reconstructor, mobility predictor, and identification recognizer during the proposed adversarial training. The encoder $Enc_L(X)$ is trained to achieve a better trade-off between sufficient task-based inference accuracy and user privacy budgets by extracting more information required by the task and less information by the privacy.
In the setting of this paper, we focus on the mobility prediction services as the next location anticipating is of great value for different applications ranging from individual-level personalized recommendation system to large-scale urban planning. We leverage the accuracy of mobility prediction to measure the $utility$ of the extracted features $Enc_L(X)$. The $privacy$ is quantified with two attackers, listed as the data reconstructor (\textit{i.e.}, information loss) and the identification recognizer (\textit{i.e.}, inaccuracy of the re-identification).

%In summarize, the assessment model consists of three important units
Hence, the proposed LSTM-AE model is composed of three crucial units, that are \textit{Mobility Prediction Unit}, \textit{Re-identification Attack Unit}, and \textit{Reconstruction Attack Unit}. We discuss the functionality of each unit before we discuss the overall performance of the model.

\textit{I. Mobility Prediction Unit}:  

\textit{i. Definition of Mobility Trajectories}: the raw GPS data or other spatial-temporal data are at least contain three elements: user identity \textit{u}, timestamps \textit{t}, location identifiers \textit{l}.
Hence, each location records \textit{r} could be denoted as \emph{$r_i$} = [\textit{$u_i$}, \textit{$t_i$}, \textit{$l_i$}], while each location sequence \emph{S} is a set of ordered location records \emph{$S_n$} =~\{\textit{r$_1$, r$_2$, r$_3$, $\cdots$, r$_n$}\}.
As for the goal of data sharing between data collects and service providers, the mobility prediction framework is deigned for a general model, which will take all users' records into consideration and make the next location prediction.
Then each location record \emph{$r_i$} here only contains \emph{$r_i$} = [\textit{$t_i$}, \textit{$l_i$}].
Therefore, given the past mobility trajectory \{\textit{r$_1$, r$_2$, r$_3$, $\cdots$, r$_n$}\}, the mobility prediction task is to estimate the most likely next location \emph{l$_n+1$} in the next time step \emph{t$_n+1$}.
%where the location is discretized into a position in a rectangular grid, a supervised classification task.
The trajectories fed into the enocder $Enc_L(X)$ are a list of location sequences \emph{S} with specific context length \emph{SL}. For instances, if the context length is 10, that indicates each sequence contains 10 history records, \emph{S} = \{r$_0$, r$_2$, r$_3$, $\cdots$, r$_9$\}, and $SL=10$.

\textit{ii. Unit Design}: 
the unit is composed of three dimensions, the input part with multi-modal embedding, the sequential part with LSTM, and a softmax output part.
As aforementioned definition, the trajectories in this work are shown as sequence \emph{S}. First, the location and timestamp are converted into one-hot vectors.
We then employ the Long-short-term memory (LSTM)~\cite{hochreiter1997long} layers to model the mobility pattern and sequential transition relation in these mobility sequences. As one of the prominent variants of the recurrent neural network, LSTM can exhibit brilliant performance on modelling entire sequences of data, especially for handling the difficulty of learning long-term dependencies with the gradient descent~\cite{zhan2019towards}.
Following the sequential module, the softmax layer outputs the probability distribution of the prediction results. This distribution is converted to the top-n accuracy metrics to illustrate the data performance.

%If a synthetic or obfuscated dataset preserves the structure of the original dataset, then its utility in the next location prediction task should be preserved. Therefore, by comparing the next location prediction accuracy of a trained model on an obfuscated dataset vs. the original, we can quantify the degradation in data utility introduced by the obfuscation technique.

\textit{II. Re-identification Attacker Unit}: 

\textit{i. Definition of Trajectory Identification}: we assumed each trajectory sequence \emph{S} is originally labeled with corresponding user identification. %and conduct user ID classification as a supervised learning task.
As each location record $r$ only contain timestamps \textit{t} and location identification \textit{l}, we leverage the user identification as the ground-truth values for the trajectory classification classes, 
which is used to classify the user \textit{u} to whom the target trajectory sequence \emph{$S_n$} = \{r$_1$, r$_2$, r$_3$, $\cdots$, r$_n$\} belongs. 


\textit{ii. Unit Design}:
the unit is composed of three dimensions, the input part with identification one-hot embedding, the sequential part with LSTM, and a softmax output part.
First, the user identification list is converted into one-hot vectors. Similar to the mobility prediction unit, the identification recognition unit also applies LSTM layers to better extract the spatio and temporal characteristics of the context. 
A softmax layer with cross-categorical entropy will be used to evaluate the recognition accuracy.
We then use the top-n accuracy for this classifier as the metrics of re-identification privacy risk (\textit{PII}); the more accurately a classifier can guess the user identification given a trajectory,
the higher the privacy risk associated with disclosing the trajectory data.
The degradation in performance of such a classifier when evaluated on a synthetic or obfuscated dataset vs. the original dataset thus serves as a measure of the effectiveness of the synthetic data generation technique at reducing privacy risk. This strategy for privacy risk assessment is demonstrated in \citeauthor{rao2020lstm} \cite{rao2020lstm}.

\textit{III. Reconstruction Attacker Unit}:
the unit is the encoder turn upside down. The unit evaluates the differences between reconstructed data $X'$ and the original one $X$ as our \textit{Privacy I}. A malicious party is free to reconstruct the data and explore any machine learning model when they have the feature extraction $Enc_L(X)$. We use an exactly layer-to-layer reverse architecture of our encoder $Enc_L$ to build a strong \textit{Reconstruction Attack Unit}. We leverage Euclidean and Manhattan distance as our metrics to measure the straightforward differences between the $X$ and $X'$.

Following the basic discussion of three units, we present the overall design of the proposed LSTM-AE model.

Our proposed privacy-preserving assessment model, the LSTM-AE, is based on representation learning and adversarial network, and aims to ease data sharing privacy concerns. 
As shown in Figure \ref{fig:proposed}, we design a multi-task adversarial network to learn a LSTM representation encoder $Enc_L$ that generate the feature representations $f=Enc_L(X)$ to optimize against the privacy disclosure risk of sensitive information, and concurrently optimize with the task accuracy (\textit{i.e.}, next location forecasting). 
Two malicious attacks, the data reconstructor and identification recognizer are attempted to retrieve sensitive information from the $Enc_L(X)$.
In particular, the encoder $Enc_L$ should satisfy high mobility prediction accuracy and high de-identification efficiency when maximizing the reconstruction loss in reversed engineering.

Given spatial-temporal raw data $\mathcal{X}$, the ground-truth label for utility (\textit{e.g.}, predictor) $y_i$,
the ground-truth label for privacy (\textit{e.g.}, identification) $z_i$, we train the LSTM encoder $Enc_L$ by adversarial learning of this multi-task network to learn the representation $\mathcal{F}=Enc_L(\mathcal{X})$. 
Specifically, when reconstructing to the data $\mathcal{X'}$, a LSTM decoder $Dec_L$ invests the features $\mathcal{F}$, that is $Dec_L: \mathcal{F}\rightarrow \mathcal{X'}$, which is trained to reconstruct the input $\mathcal{X}$ from features $\mathcal{F}$ by minimizing the reconstruction loss:
\begin{equation}
   \mathcal{L_R} = \| Dec_L(\mathcal{F}) - \mathcal{X}\|^2
\end{equation}
where $ Dec_L(\mathcal{F}) = \mathcal{X'}$, the reconstructed data.
Then the extracted encoder features $\mathcal{F}$ is fed into two discriminators, respectively. 

The next location predictor, that is the utility discriminator $U_D$, is trained to output a probability over the Y potential location classes for each trajectory.
Discriminative training in the utility discriminator is to maximize the prediction accuracy, telling the cross-entropy error $\epsilon$ by minimizing the following loss:
\begin{equation}
    \mathcal{L_U} = -\sum_{i=1}^{\mathbf{Y}} y_i\text{log}(U_D(\mathcal{F}))
\end{equation}
where $y_i$ is the ground-truth label for utility, $U_D(\mathcal{F})$ represents the predicted class by the next location predictor.

The identification recognizer, that is the privacy discriminator $P_D$, is trained to
classify the trajectory into different user categories. Then in this privacy discriminator,
the cross entropy loss is minimized by the loss:
\begin{equation}
    \mathcal{L_P} = -\sum_{i=1}^{\mathbf{Z}} z_i\text{log}(P_D(\mathcal{F}))
\end{equation}
where $z_i$ is the ground-truth value for privacy, $P_D(\mathcal{F})$ represents the predicted identification class by the identification recognizer.

The overall training is to achieve privacy-utility trade-off by adversarial learning on $\mathcal{L_R}$, $\mathcal{L_U}$, and $\mathcal{L_P}$, where the training objective can be written as:
\begin{equation}
\begin{aligned}
    \text{Min} \left(\mathcal{L}_{sum}\right) & = -\lambda_1 \mathcal{L_R} + \lambda_2 \mathcal{L_U} - \lambda_3 \mathcal{L_P} \\ 
    &= - \lambda_1 * \| Dec_L(\mathcal{F}) - \mathcal{X}\|^2 + \lambda_2 * (-\sum_{i=1}^{\mathbf{Y}} y_i\text{log}(U_D(\mathcal{F}))) - \lambda_3 * (-\sum_{i=1}^{\mathbf{Z}} z_i\text{log}(P_D(\mathcal{F})))
\end{aligned}
\label{equ:sumloss}
\end{equation}

The gradient of the loss then back-propagate through the LSTM network to guide the training of the encoder $Enc_L(X)$.
The encoder is updated with the loss function until convergence.

The LSTM-AE model is the core component of the \textit{Model Assessment Module}, it could be utilized to evaluate the utility and privacy level of any dataset. At the same time, it also could be utilized as an independent model to attain a privacy-preserving feature representation \textit{f} for data sharing. This transformation is controlled by the new designed loss function, the Equation~\ref{equ:sumloss} with $\lambda_1$, $\lambda_2$ and $\lambda_3$. They are Lagrange multipliers~\cite{beavis1990optimisation} that are utilized to find a maxima or minima of a constrained problem. When two of them are set to zero, the model is transformed to a specific evaluation tool for specific data and a specific task.
When three multipliers are utilized in a collaboration way, it controls the relative importance of each unit and then conducts the overall model to find the maxima or minima of the specific trade-offs.
 
\subsubsection{Evaluation Method}

We utilize the framework to train and assess our model in comparison to a benchmark model, by first utilizing a trained generative model to produce synthetic or otherwise geo-masked data,
and then comparing performance metrics on the original dataset vs. the synthetic dataset, to assess the relative decline in utility vs. privacy introduced by the data generation process.
We utilize the framework to compare the utility (via next location prediction accuracy) and privacy (via user identification classification) of our LSTM-AE model with that of the LSTM-TrajGAN \cite{rao2020lstm} model.
Section 4 of this paper details the results of this comparison.

%\subsubsection{Mobility Prediction Performance}
%\subsubsection{Identification Recognition Performance}
%\textbf{Unicity Test:} 


==> 4_evaluation/table_compare2.tex <==

\begin{table*}[]
   \centering
   \begin{tabular}{cccccccccc}
    \hline
    \multirow{2}{*}{\shortstack{Comparison}} & \multirow{2}{*}{\shortstack{Datasets}}  & \multicolumn{2}{|c|}{Similarity Index} & \multicolumn{3}{c|}{Utility (\% for decline)} & \multicolumn{3}{c}{Privacy (\% for gain)} \\
    \cline{3-10}
        &  & \multicolumn{1}{|c}{Euc(log)} & \multicolumn{1}{c|}{Man(log)} & top-1  & top-3  & \multicolumn{1}{c|}{top-5} & top-1  & top-3 & top-5 \\
        \hline
        \multirow{4}{*}{\shortstack{Standalone\\Model}} & mdc & 0.001 & 0.002 & 0.9347  & 0.9837  & 0.9922 & 0.9247 & 0.9819 & 0.9911\\
        %\cline{2-12}
        &privamov & 1.281 & 2.554 & 0.9482  & 0.9878 & 0.9954 & 0.5643 & 0.8215 & 0.8765 \\
        %\cline{2-12}
        &geolife & & & 0.4705 & 0.6842 & 0.7636 & 0.6572 & 0.8690 & 0.9294\\
        %\cline{2-12}
        &foursquare & 2.357 & 4.464 & 0.6468 & 0.8210 & 0.8823 & 0.8780 & 0.9735 & 0.9892 \\
        %\cline{2-12}
        \hline
        \multirow{4}{*}{\shortstack{Traj-GAN}} & mdc & 3.526 & 5.456  & -46.32\% & -24.16\% & -15.98\% & 20.32\% & 8.13\% & 4.02\% \\
        %\cline{2-12}
        &privamov & 3.704 & 5.779 & -6.60\% & -1.89\% & -0.93\% & 14.17\% & 14.35\% & 8.88\%\\
        %\cline{2-12}
        &geolife & 4.581 & 6.680 & -62.31\% & -50.45\% & -43.72\% & \% & \% & \% \\
        %\cline{2-12}
        &foursquare & 4.795 & 6.710 & -26.30\% & -22.30\% & -18.75\% & 51.86\% & 32.49\% & 23.49\% \\
        %\cline{2-12}
        \hline
        \multirow{4}{*}{\shortstack{Proposed\\Model}} & mdc & & &  &  &  &  &  & \\
        %\cline{2-12}
        &privamov & & &   &  &  &  &  & \\
        %\cline{2-12}
        &geolife & & &   &  &  &  &  &\\
        %\cline{2-12}
        &foursquare & & &  &  &  &  &  &\\
        %\cline{2-12}
        \hline
        
    \end{tabular}
    \caption{}
    \label{tab:compare}
\end{table*}

\begin{table*}[]
   \centering
   \begin{tabular}{cccccccccc}
    \hline
    \multirow{2}{*}{\shortstack{Datasets}} & \multirow{2}{*}{\shortstack{Models}}  & \multicolumn{2}{|c|}{Similarity Index} & \multicolumn{3}{c|}{Utility (\% for decline)} & \multicolumn{3}{c}{Privacy (\% for gain)} \\
    \cline{3-10}
        &  & \multicolumn{1}{|c}{Euc(log)} & \multicolumn{1}{c|}{Man(log)} & top-1  & top-3  & \multicolumn{1}{c|}{top-5} & top-1  & top-3 & top-5 \\
        \hline
        \multirow{3}{*}{\shortstack{MDC}} & Standalone Model & 0.001 & 0.002 & 0.9347  & 0.9837  & 0.9922 & 0.9247 & 0.9819 & 0.9911\\
        & Traj-GAN & 3.526 & 5.456  & -46.32\% & -24.16\% & -15.98\% & 20.32\% & 8.13\% & 4.02\% \\
        & Proposed Model & \textbf{3.732} & \textbf{6.023} & \textbf{-13.43\%} & \textbf{-6.26\%} & \textbf{-3.95\%} & \textbf{65.51\%} & \textbf{45.11\%} & \textbf{34.86\%} \\
        \hline
        \multirow{3}{*}{\shortstack{Priva'Mov}} & Standalone Model & 1.281 & 2.554 & 0.9482  & 0.9878 & 0.9954 & 0.5643 & 0.8215 & 0.8765 \\
        & Traj-GAN & 3.704 & 5.779 & \textbf{-6.60\%} & \textbf{-1.89\%} & \textbf{-0.93\%} & 14.17\% & 14.35\% & 8.88\%\\
        & Proposed Model & \textbf{4.164} & \textbf{5.803} & -10.81\% & -6.83\% & -4.91\% & \textbf{35.29\%} & \textbf{14.97\%} & \textbf{10.05\%} \\
        \hline
        
        \multirow{3}{*}{\shortstack{Geolife}} & Standalone Model & 1.903 & 3.804 & 0.4705 & 0.6842 & 0.7636 & 0.6572 & 0.8690 & 0.9294\\
        & Traj-GAN & 4.581 & 6.680 & -62.31\% & -50.45\% & -43.72\% & \textbf{66.73\%} & \textbf{47.89\%} & \textbf{37.22\%} \\
        & Proposed Model & \textbf{4.616}& \textbf{6.928}& \textbf{-21.13\%} & \textbf{-18.78\%} & \textbf{-17.11\%} & 55.49\% & 40.40\% & 32.34\% \\
        
        \hline
        \multirow{3}{*}{\shortstack{FourSquare}} & Standalone Model & 2.357 & 4.464 & 0.6468 & 0.8210 & 0.8823 & 0.8780 & 0.9735 & 0.9892 \\
        & Traj-GAN & \textbf{4.795} & \textbf{6.710} & -26.30\% & -22.30\% & -18.75\% & \textbf{51.86\%} & 32.49\% & 23.49\% \\
        & Proposed Model & 4.541 & 6.638 & \textbf{-2.54\%} & \textbf{-3.14\%} & \textbf{-2.84\%} & \textbf{51.08\%} & \textbf{34.39\%} & \textbf{26.16\%}\\
        \hline
        
    \end{tabular}
    \caption{Performance comparison between our proposed model with standalone model and the Traj-GAN model. The results show in this table are all with sequence length 10 (that is $SL=10$). The similarity indexes (Euclidean and Manhattan distance) are leveraged to intuitively represent the difference between the original data and reconstructed data. The \textit{Utility} and \textit{Privacy} columns of Standalone Model represent the original prediction and re-identification capability of the separated units without consideration of utility-privacy tradeoffs, respectively. The utility in \% represents the utility declines with different frameworks, and the privacy in \% represents the privacy gains. Noted that the identification accuracy is leveraged as the privacy metric here, while the privacy gain is calculated by the re-identification error.}
    \label{tab:compare}
\end{table*}
